Data-Efficient Framework for Real-world Multiple Sound Source 2D Localization

Deep neural networks have recently led to promising results for the task of multiple sound source localization. Yet, they require a lot of training data to cover a variety of acoustic conditions and microphone array layouts. One can leverage acoustic simulators to inexpensively generate labeled training data. However, models trained on synthetic data tend to perform poorly with real-world recordings due to the domain mismatch. Moreover, learning for different microphone array layouts makes the task more complicated due to the infinite number of possible layouts. We propose to use adversarial learning methods to close the gap between synthetic and real domains. Our novel ensemble-discrimination method significantly improves the localization performance without requiring any label from the real data. Furthermore, we propose a novel explicit transformation layer to be embedded in the localization architecture. It enables the model to be trained with data from specific microphone array layouts while generalizing well to unseen layouts during inference.

==> tables/discriminator.tex <==
\begin{table}[bt]
\footnotesize\addtolength{\tabcolsep}{-5pt}
\begin{center}
\caption{Discriminators detailed architecture}
\label{tab:discriminator}
\begin{tabular}{ccccc}
\cline{4-5}
                                      &                                  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Layer}                        & \multicolumn{1}{c|}{Output size}            \\ \cline{4-5} 
                                      &                                  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Input}                        & \multicolumn{1}{c|}{1$\times$81$\times$81}  \\ \cline{1-2}
\multicolumn{1}{|c|}{Layer}           & \multicolumn{1}{c|}{Output size} & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Conv(7$\times$7) + BN + ReLU} & \multicolumn{1}{c|}{32$\times$27$\times$27} \\ \cline{1-2}
\multicolumn{1}{|c|}{Input}           & \multicolumn{1}{c|}{1024}        & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Conv(7$\times$7) + BN + ReLU} & \multicolumn{1}{c|}{64$\times$9$\times$9}   \\
\multicolumn{1}{|c|}{Dense + ReLU}    & \multicolumn{1}{c|}{512}         & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Conv(5$\times$5) + BN + ReLU} & \multicolumn{1}{c|}{128$\times$4$\times$4}  \\
\multicolumn{1}{|c|}{Dense + ReLU}    & \multicolumn{1}{c|}{16}          & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Conv(3$\times$3) + BN + ReLU} & \multicolumn{1}{c|}{128$\times$2$\times$2}  \\
\multicolumn{1}{|c|}{Dense + ReLU}    & \multicolumn{1}{c|}{4}           & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Reshape}                      & \multicolumn{1}{c|}{512}                    \\
\multicolumn{1}{|c|}{Dense + Sigmoid} & \multicolumn{1}{c|}{1}           & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Dense + ReLU}                 & \multicolumn{1}{c|}{16}                     \\ \cline{1-2}
\multicolumn{2}{c}{\textit{Intermediate discriminator}}                                            & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Dense + ReLU}                 & \multicolumn{1}{c|}{4}                      \\
                                      &                                  & \multicolumn{1}{c|}{} & \multicolumn{1}{c|}{Dense + Sigmoid}              & \multicolumn{1}{c|}{1}                      \\ \cline{4-5} 
\multicolumn{2}{c}{}                                                     &                       & \multicolumn{2}{c}{\textit{Output discriminator}}                                                                  
\end{tabular}
\end{center}
\normalsize
\end{table}


==> tables/results.tex <==
\begin{table}[bt]
\footnotesize\addtolength{\tabcolsep}{-5pt}
\begin{center}
\caption{Domain adaptation results}
\label{tab:results}
\begin{tabular}{cc|cccc|cccc|}
\cline{3-10}
                                                    &           & \multicolumn{4}{c|}{TestRc}                                                                                                          & \multicolumn{4}{c|}{TestRj}                                                                                                          \\ \hline
\multicolumn{2}{|c|}{Method}                                    & \multicolumn{1}{c|}{Pre} & \multicolumn{1}{c|}{Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{F1$\uparrow$}} & \cellcolor[HTML]{EFEFEF}{\tiny RMSE}$\downarrow$ & \multicolumn{1}{c|}{Pre} & \multicolumn{1}{c|}{Rec} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}{F1$\uparrow$}} & \cellcolor[HTML]{EFEFEF}{\tiny RMSE}$\downarrow$ \\ \hline
\multicolumn{1}{|c|}{}                              & S         & .83                      & .44                      & \cellcolor[HTML]{EFEFEF}.57                     & \cellcolor[HTML]{EFEFEF}.48  & .85                      & .51                      & \cellcolor[HTML]{EFEFEF}.64                     & \cellcolor[HTML]{EFEFEF}.40  \\ \cline{2-2}
\multicolumn{1}{|c|}{\multirow{-2}{*}{Lower bound}} & S+        & .80                      & .55                      & \cellcolor[HTML]{EFEFEF}.65                     & \cellcolor[HTML]{EFEFEF}.43  & .90                      & .60                      & \cellcolor[HTML]{EFEFEF}.72                     & \cellcolor[HTML]{EFEFEF}.39  \\ \hline
\multicolumn{1}{|c|}{}                              & R         & .96                      & .69                      & \cellcolor[HTML]{EFEFEF}.80                     & \cellcolor[HTML]{EFEFEF}.24  & .92                      & .54                      & \cellcolor[HTML]{EFEFEF}.68                     & \cellcolor[HTML]{EFEFEF}.37  \\ \cline{2-2}
\multicolumn{1}{|c|}{\multirow{-2}{*}{Upper bound}} & R\&S      & .91                      & .76                      & \cellcolor[HTML]{EFEFEF}.83                     & \cellcolor[HTML]{EFEFEF}.33  & .96                      & .78                      & \cellcolor[HTML]{EFEFEF}.86                     & \cellcolor[HTML]{EFEFEF}.30  \\ \hline
\multicolumn{1}{|c|}{}                              & GRint      & .89                      & .56                      & \cellcolor[HTML]{EFEFEF}.69                     & \cellcolor[HTML]{EFEFEF}.38  & .92                      & .66                      & \cellcolor[HTML]{EFEFEF}.77                     & \cellcolor[HTML]{EFEFEF}.36  \\ \cline{2-2}
\multicolumn{1}{|c|}{}                              & LFint      & .90                        & .62                        & \cellcolor[HTML]{EFEFEF}.73                       & \cellcolor[HTML]{EFEFEF}.45    & .92                        & .70                        & \cellcolor[HTML]{EFEFEF}.79                       & \cellcolor[HTML]{EFEFEF}.41    \\ \cline{2-2}
\multicolumn{1}{|c|}{}                              & GRout      & .79                      & .71                      & \cellcolor[HTML]{EFEFEF}.75                     & \cellcolor[HTML]{EFEFEF}.43  & .88                      & .80                      & \cellcolor[HTML]{EFEFEF}.84                     & \cellcolor[HTML]{EFEFEF}.41  \\ \cline{2-2}
\multicolumn{1}{|c|}{}                              & LFout      & .80                      & .70                      & \cellcolor[HTML]{EFEFEF}.75                     & \cellcolor[HTML]{EFEFEF}.46  & .86                      & .74                      & \cellcolor[HTML]{EFEFEF}.80                     & \cellcolor[HTML]{EFEFEF}.45  \\ \cline{2-2}
\multicolumn{1}{|c|}{}                              & GRintGRout  & .86                      & .73                      & \cellcolor[HTML]{EFEFEF}.79                     & \cellcolor[HTML]{EFEFEF}.41  & .91                      & .79                      & \cellcolor[HTML]{EFEFEF}.85                     & \cellcolor[HTML]{EFEFEF}.37  \\ \cline{2-2}
\multicolumn{1}{|c|}{\multirow{-6}{*}{Adv. Adap.}}  & GRintGRout+ & .85                      & .74                      & \cellcolor[HTML]{EFEFEF}.79                     & \cellcolor[HTML]{EFEFEF}.42  & .88                      & .76                      & \cellcolor[HTML]{EFEFEF}.81                     & \cellcolor[HTML]{EFEFEF}.39  \\ \hline
\end{tabular}
\end{center}
\end{table}


==> tables/results0.tex <==
% \usepackage{colortbl}
% \usepackage{multirow}
% \usepackage{hhline}

\begin{table*}
\footnotesize\addtolength{\tabcolsep}{-6pt}
\begin{center}
\caption{Domain Adaptation Results.}
\label{tab:results0} %https://tex.stackexchange.com/a/59805
%%%%%%%%%%%%%%%%%%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hhline{~~|--------|~|--------|} 
%\cline{3-10}\cline{12-19}
\multicolumn{2}{c|}{}                                    & \multicolumn{8}{c|}{\textbf{TestRc (classical \& funk)}}                                                                                                                                                                                                    &  & \multicolumn{8}{c|}{\textbf{TestRj (jazz)}}                                                                                                                                                                                                                  \\ 
\hhline{|--|--|--|--|--|~|--|--|--|--|}
\multicolumn{2}{|c|}{\textbf{Method}}                    & \multicolumn{2}{c|}{\textbf{RMSE $\downarrow$}} & \multicolumn{2}{c|}{\textbf{Precision $\uparrow$}} & \multicolumn{2}{c|}{\textbf{Recall $\uparrow$}} & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}\textbf{F1-Score $\uparrow$}}                          &  & \multicolumn{2}{c|}{\textbf{RMSE $\downarrow$}} & \multicolumn{2}{c|}{\textbf{Precision $\uparrow$}} & \multicolumn{2}{c|}{\textbf{Recall $\uparrow$}} & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}\textbf{F1-Score $\uparrow$}}                           \\ 
\hhline{|-|-|--|--|--|--|~|--|--|--|--|}
Low B.                              & S                  & \multicolumn{2}{c|}{.51$\pm$.01}                 & \multicolumn{2}{c|}{.80$\pm$.03}                    & \multicolumn{2}{c|}{.48$\pm$.03}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}.60$\pm$.02}                                            &  & \multicolumn{2}{c|}{.45$\pm$.01}                 & \multicolumn{2}{c|}{.83$\pm$.02}                    & \multicolumn{2}{c|}{.51$\pm$.02}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}.63$\pm$.01}                                             \\ 
\hhline{|-|-|--|--|--|--|~|--|--|--|--|}
Up B.                               & R                  & \multicolumn{2}{c|}{.34$\pm$.01}                 & \multicolumn{2}{c|}{.95$\pm$.03}                    & \multicolumn{2}{c|}{.71$\pm$.03}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}.81$\pm$.01}                                            &  & \multicolumn{2}{c|}{.36$\pm$.01}                 & \multicolumn{2}{c|}{.93$\pm$.01}                    & \multicolumn{2}{c|}{.66$\pm$.03}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}.77$\pm$.02}                                             \\ 
\hhline{|-|-|--|--|--|--|~|--|--|--|--|}
\multirow{2}{*}{Others}             & R\&S               & \multicolumn{2}{c|}{.33$\pm$.02}                 & \multicolumn{2}{c|}{.96$\pm$.03}                    & \multicolumn{2}{c|}{.71$\pm$.04}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}.82$\pm$.02}                                            &  & \multicolumn{2}{c|}{.30$\pm$.01}                 & \multicolumn{2}{c|}{.98$\pm$.01}                    & \multicolumn{2}{c|}{.70$\pm$.06}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}.81$\pm$.04}                                             \\ 
\hhline{|~|-|--|--|--|--|~|--|--|--|--|}
                                    & S+                 & \multicolumn{2}{c|}{.44$\pm$.00}                 & \multicolumn{2}{c|}{.84$\pm$.01}                    & \multicolumn{2}{c|}{.57$\pm$.01}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}.68$\pm$.01}                                            &  & \multicolumn{2}{c|}{.40$\pm$.01}                 & \multicolumn{2}{c|}{.89$\pm$.01}                    & \multicolumn{2}{c|}{.62$\pm$.02}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.878,0.878,0.878}}.73$\pm$.02}                                             \\ 
\hhline{|-|-|--|--|--|--|~|--|--|--|--|}
%\cline{1-10}\cline{12-19}
\multicolumn{2}{|c|}{\textit{\textbf{Stopping Epoch}}}   & \textit{200th} & \textit{Sel.}               & \textit{200th}   & \textit{Sel.}                & \textit{200th}   & \textit{Sel.}             & \textit{200th}                                       & \textit{Sel.}                                        &  & \textit{200th} & \textit{Sel.}               & \textit{200th}   & \textit{Sel.}                & \textit{200th}   & \textit{Sel.}             & \textit{200th}                                       & \textit{Sel.}                                         \\ 
\hhline{|-|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Adv.\\Adap.\end{tabular}} & G\ts{r}int              & .48$\pm$.03        & .42$\pm$.02                     & .81$\pm$.05          & .86$\pm$.02                      & .57$\pm$.04          & .60$\pm$.04                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.67$\pm$.02          & {\cellcolor[rgb]{0.878,0.878,0.878}}.71$\pm$.02          &  & .45$\pm$.03        & .40$\pm$.01                     & .86$\pm$.04          & .92$\pm$.01                      & .59$\pm$.06          & .67$\pm$.04                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.70$\pm$.04          & {\cellcolor[rgb]{0.878,0.878,0.878}}.77$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                    & L\ts{f}int              & .50$\pm$.03        & .46$\pm$.03                     & .71$\pm$.06          & .81$\pm$.04                      & .44$\pm$.09          & .53$\pm$.03                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.53$\pm$.08          & {\cellcolor[rgb]{0.878,0.878,0.878}}.64$\pm$.03          &  & .47$\pm$.01        & .46$\pm$.03                     & .79$\pm$.04          & .86$\pm$.04                      & .44$\pm$.13          & .57$\pm$.04                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.56$\pm$.12          & {\cellcolor[rgb]{0.878,0.878,0.878}}.69$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                    & G\ts{r}out              & .51$\pm$.02        & .48$\pm$.01                     & .68$\pm$.02          & .78$\pm$.04                      & .67$\pm$.02          & .67$\pm$.04                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.67$\pm$.02          & {\cellcolor[rgb]{0.878,0.878,0.878}}.72$\pm$.03          &  & .51$\pm$.03        & .47$\pm$.01                     & .77$\pm$.03          & .84$\pm$.06                      & .75$\pm$.03          & .75$\pm$.04                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.76$\pm$.03          & {\cellcolor[rgb]{0.878,0.878,0.878}}.79$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                    & L\ts{f}out              & .51$\pm$.02        & .47$\pm$.02                     & .64$\pm$.04          & .79$\pm$.04                      & .67$\pm$.02          & .68$\pm$.02                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.65$\pm$.03          & {\cellcolor[rgb]{0.878,0.878,0.878}}.73$\pm$.02          &  & .51$\pm$.03        & .46$\pm$.01                     & .71$\pm$.05          & .87$\pm$.03                      & .75$\pm$.04          & .74$\pm$.03                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.73$\pm$.04          & {\cellcolor[rgb]{0.878,0.878,0.878}}.80$\pm$.01           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                    & G\ts{r}intG\ts{r}out         & .47$\pm$.05        & .43$\pm$.03                     & \textbf{.82$\pm$.05} & .86$\pm$.04                      & \textbf{.72$\pm$.03} & .73$\pm$.02                   & {\cellcolor[rgb]{0.878,0.878,0.878}}\textbf{.76$\pm$.02} & {\cellcolor[rgb]{0.878,0.878,0.878}}\textbf{.79$\pm$.01} &  & .46$\pm$.03        & .41$\pm$.02                     & \textbf{.88$\pm$.03} & .91$\pm$.02                      & .77$\pm$.03          & \textbf{.79$\pm$.03}          & {\cellcolor[rgb]{0.878,0.878,0.878}}\textbf{.82$\pm$.01} & {\cellcolor[rgb]{0.878,0.878,0.878}}.84$\pm$.01           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                    & L\ts{f}intL\ts{f}out         & .53$\pm$.03        & .46$\pm$.03                     & .65$\pm$.10          & .83$\pm$.03                      & .60$\pm$.09          & .68$\pm$.05                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.62$\pm$.10          & {\cellcolor[rgb]{0.878,0.878,0.878}}.74$\pm$.03          &  & .51$\pm$.01        & .45$\pm$.03                     & .69$\pm$.12          & .88$\pm$.02                      & .61$\pm$.13          & .75$\pm$.04                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.65$\pm$.12          & {\cellcolor[rgb]{0.878,0.878,0.878}}.81$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                    & G\ts{r}intG\ts{r}out+        & .46$\pm$.02        & .42$\pm$.01                     & .76$\pm$.07          & \textbf{.88$\pm$.03}             & .71$\pm$.05          & .71$\pm$.06                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.73$\pm$.02          & {\cellcolor[rgb]{0.878,0.878,0.878}}.78$\pm$.02          &  & .45$\pm$.02        & .39$\pm$.02                     & .85$\pm$.06          & \textbf{.95$\pm$.02}             & \textbf{.78$\pm$.05} & .77$\pm$.05                   & {\cellcolor[rgb]{0.878,0.878,0.878}}.81$\pm$.03          & {\cellcolor[rgb]{0.878,0.878,0.878}}\textbf{.85$\pm$.03}  \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                    & L\ts{f}intL\ts{f}out+        & .50$\pm$.02        & .43$\pm$.01                     & .72$\pm$.09          & .86$\pm$.05                      & .65$\pm$.02          & \textbf{.74$\pm$.02}          & {\cellcolor[rgb]{0.878,0.878,0.878}}.68$\pm$.03          & {\cellcolor[rgb]{0.878,0.878,0.878}}\textbf{.79$\pm$.02} &  & .49$\pm$.02        & .41$\pm$.03                     & .80$\pm$.08          & .89$\pm$.03                      & .71$\pm$.03          & \textbf{.79$\pm$.01}          & {\cellcolor[rgb]{0.878,0.878,0.878}}.75$\pm$.03          & {\cellcolor[rgb]{0.878,0.878,0.878}}.84$\pm$.01          \\
\hhline{|----------~--------|}
%\hhline{|-|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
\end{tabular}
%%%%%%%%%%%%%%%%%%
\begin{scriptsize}
\newline
\begin{center}
\vspace{-1.4em}
\textit{Low B.}, \textit{Up B.}, \textit{Adv. Adap.}, and \textit{Sel.} is
short for lower, upper bound, adversarial adaptation, and model selection 
respectively; $\uparrow$/$\downarrow$ represent the higher/lower is better 
respectively.
\end{center}
\end{scriptsize}
\end{center}
\vspace{-1.0em}
\normalsize
\end{table*}



==> tables/results0_.tex <==
% \usepackage{colortbl}
% \usepackage{multirow}
% \usepackage{hhline}
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|} 
\hline
\multicolumn{2}{|c|}{\textbf{Method}}                                               & \multicolumn{2}{c|}{\textbf{RMSE\textbf{ ↓}}} & \multicolumn{2}{c|}{\textbf{Precision ↑}} & \multicolumn{2}{c|}{\textbf{Recall\textbf{ ↑}}} & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.843,0.843,0.843}}\textbf{F1-Score\textbf{ ↑}}}                        \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Lower\\Bound\end{tabular}} & S           & \multicolumn{2}{c|}{.51±.01}                  & \multicolumn{2}{c|}{.80±.03}              & \multicolumn{2}{c|}{.48±.03}                    & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.851,0.851,0.851}}.60±.02}                                             \\ 
\hhline{|~|-|--|--|--|--|}
                                                                      & S+          & \multicolumn{2}{c|}{.44±.00}                  & \multicolumn{2}{c|}{.84±.01}              & \multicolumn{2}{c|}{.57±.01}                    & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.851,0.851,0.851}}.68±.01}                                             \\ 
\hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Upper\\Bound\end{tabular}} & R           & \multicolumn{2}{c|}{.34±.01}                  & \multicolumn{2}{c|}{.95±.03}              & \multicolumn{2}{c|}{.71±.03}                    & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.851,0.851,0.851}}.81±.01}                                             \\ 
\hhline{|~|-|--|--|--|--|}
                                                                      & R\&S        & \multicolumn{2}{c|}{.33±.02}                  & \multicolumn{2}{c|}{.96±.03}              & \multicolumn{2}{c|}{.71±.04}                    & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.851,0.851,0.851}}.82±.02}                                             \\ 
\hline
\multicolumn{2}{|c|}{\textbf{\textit{Stopping Epoch}}}                              & \textit{200th} & \textit{Best}                & \textit{200th}   & \textit{Best}          & \textit{200th}   & \textit{Best}                & \textit{200th}                                       & \textit{Best}                                         \\ 
\hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Adv.\\Adap.\end{tabular}}  & GRint       & .48±.03        & .42±.02                      & .81±.05          & .86±.02                & .57±.04          & .60±.04                      & {\cellcolor[rgb]{0.847,0.847,0.847}}.67±.02          & {\cellcolor[rgb]{0.847,0.847,0.847}}.71±.02           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|}
                                                                      & LFint       & .50±.03        & .46±.03                      & .71±.06          & .81±.04                & .44±.09          & .53±.03                      & {\cellcolor[rgb]{0.847,0.847,0.847}}.53±.08          & {\cellcolor[rgb]{0.847,0.847,0.847}}.64±.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|}
                                                                      & GRout       & .51±.02        & .48±.01                      & .68±.02          & .78±.04                & .67±.02          & .67±.04                      & {\cellcolor[rgb]{0.847,0.847,0.847}}.67±.02          & {\cellcolor[rgb]{0.847,0.847,0.847}}.72±.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|}
                                                                      & LFout       & .51±.02        & .47±.02                      & .64±.04          & .79±.04                & .67±.02          & .68±.02                      & {\cellcolor[rgb]{0.847,0.847,0.847}}.65±.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}.73±.02           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|}
                                                                      & GRintGRout  & .47±.05        & .43±.03                      & \textbf{.82±.05} & .86±.04                & \textbf{.72±.03} & .73±.02                      & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.76±.02} & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.79±.01}  \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|}
                                                                      & LFintLFout  & .53±.03        & .46±.03                      & .65±.10          & .83±.03                & .60±.09          & .68±.05                      & {\cellcolor[rgb]{0.847,0.847,0.847}}.62±.10          & {\cellcolor[rgb]{0.847,0.847,0.847}}.74±.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|}
                                                                      & GRintGRout+ & .46±.02        & \textbf{.}42±.0\textbf{1}    & .76±.07          & \textbf{.88±.03}       & .71±.05          & .71±.06                      & {\cellcolor[rgb]{0.847,0.847,0.847}}.73±.02          & {\cellcolor[rgb]{0.847,0.847,0.847}}.78±.02           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|}
                                                                      & LFintLFout+ & .50±.02        & .43±.01                      & .72±.09          & .86±.05                & .65±.02          & \textbf{.74±.02}             & {\cellcolor[rgb]{0.847,0.847,0.847}}.68±.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.79±.02}  \\
\hline
\end{tabular}
\end{table}


==> tables/results0__.tex <==
% \usepackage{colortbl}
% \usepackage{multirow}
% \usepackage{hhline}


\begin{table*}
\footnotesize\addtolength{\tabcolsep}{-5pt}
\centering
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|l|c|c|c|c|} 
\cline{3-10}\cline{12-15}
\multicolumn{2}{c|}{\textbf{}}                                                      & \multicolumn{8}{c|}{\textbf{TestRc (classical \& funk)} }                                                                                                                                                                               &  & \multicolumn{4}{c|}{\textbf{TestRj (jazz)}}                                                                                                         \\ 
\hhline{|--|--|--|--|--|~|--|--|}
\multicolumn{2}{|c|}{\textbf{Method}}                                               & \multicolumn{2}{c|}{\textbf{RMSE$\downarrow$}} & \multicolumn{2}{c|}{\textbf{Precision$\uparrow$}} & \multicolumn{2}{c|}{\textbf{Recall$\uparrow$}} & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{F1-Score$\uparrow$} }                               &  & \multicolumn{2}{c|}{\textbf{RMSE$\downarrow$}} & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{F1-Score$\uparrow$}}                                 \\ 
\hhline{|-|-|--|--|--|--|~|--|--|}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Lower\\Bound\end{tabular}} & S           & \multicolumn{2}{c|}{.51$\pm$.01}         & \multicolumn{2}{c|}{.80$\pm$.03}              & \multicolumn{2}{c|}{.48$\pm$.03}           & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.60$\pm$.02}                                            &  & \multicolumn{2}{c|}{.45$\pm$.01}         & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.63$\pm$.01}                                             \\ 
\hhline{|~|-|--|--|--|--|~|--|--|}
                                                                      & S+          & \multicolumn{2}{c|}{.44$\pm$.00}         & \multicolumn{2}{c|}{.84$\pm$.01}              & \multicolumn{2}{c|}{.57$\pm$.01}           & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.68$\pm$.01}                                            &  & \multicolumn{2}{c|}{.40$\pm$.01}         & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.73$\pm$.02}                                             \\ 
\hhline{|-|-|--|--|--|--|~|--|--|}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Upper\\Bound\end{tabular}} & R           & \multicolumn{2}{c|}{.34$\pm$.01}         & \multicolumn{2}{c|}{.95$\pm$.03}              & \multicolumn{2}{c|}{.71$\pm$.03}           & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.81$\pm$.01}                                            &  & \multicolumn{2}{c|}{.36$\pm$.01}         & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.77$\pm$.02}                                             \\ 
\hhline{|~|-|--|--|--|--|~|--|--|}
                                                                      & R\&S        & \multicolumn{2}{c|}{.33$\pm$.02}         & \multicolumn{2}{c|}{.96$\pm$.03}              & \multicolumn{2}{c|}{.71$\pm$.04}           & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.82$\pm$.02}                                            &  & \multicolumn{2}{c|}{.30$\pm$.01}         & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.81$\pm$.04}                                             \\ 
\cline{1-10}\cline{12-15}
\multicolumn{2}{|c|}{\textit{\textbf{Stopping Epoch}}}                              & \textit{200th} & \textit{Sel.}       & \textit{200th}   & \textit{Sel.}          & \textit{200th}   & \textit{Sel.}       & \textit{200th}                                       & \textit{Sel.}                                        &  & \textit{200th} & \textit{Sel.}       & \textit{200th}                                       & \textit{Sel.}                                         \\ 
\hhline{|-|-|-|-|-|-|-|-|-|-|~|-|-|-|-|}
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Adv.\\Adap.\end{tabular}}  & GRint       & .48$\pm$.03        & .42$\pm$.02             & .81$\pm$.05          & .86$\pm$.02                & .57$\pm$.04          & .60$\pm$.04             & {\cellcolor[rgb]{0.847,0.847,0.847}}.67$\pm$.02          & {\cellcolor[rgb]{0.847,0.847,0.847}}.71$\pm$.02          &  & .45$\pm$.03        & .40$\pm$.01             & {\cellcolor[rgb]{0.847,0.847,0.847}}.70$\pm$.04          & {\cellcolor[rgb]{0.847,0.847,0.847}}.77$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|}
                                                                      & LFint       & .50$\pm$.03        & .46$\pm$.03             & .71$\pm$.06          & .81$\pm$.04                & .44$\pm$.09          & .53$\pm$.03             & {\cellcolor[rgb]{0.847,0.847,0.847}}.53$\pm$.08          & {\cellcolor[rgb]{0.847,0.847,0.847}}.64$\pm$.03          &  & .47$\pm$.01        & .46$\pm$.03             & {\cellcolor[rgb]{0.847,0.847,0.847}}.56$\pm$.12          & {\cellcolor[rgb]{0.847,0.847,0.847}}.69$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|}
                                                                      & GRout       & .51$\pm$.02        & .48$\pm$.01             & .68$\pm$.02          & .78$\pm$.04                & .67$\pm$.02          & .67$\pm$.04             & {\cellcolor[rgb]{0.847,0.847,0.847}}.67$\pm$.02          & {\cellcolor[rgb]{0.847,0.847,0.847}}.72$\pm$.03          &  & .51$\pm$.03        & .47$\pm$.01             & {\cellcolor[rgb]{0.847,0.847,0.847}}.76$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}.79$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|}
                                                                      & LFout       & .51$\pm$.02        & .47$\pm$.02             & .64$\pm$.04          & .79$\pm$.04                & .67$\pm$.02          & .68$\pm$.02             & {\cellcolor[rgb]{0.847,0.847,0.847}}.65$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}.73$\pm$.02          &  & .51$\pm$.03        & .46$\pm$.01             & {\cellcolor[rgb]{0.847,0.847,0.847}}.73$\pm$.04          & {\cellcolor[rgb]{0.847,0.847,0.847}}.80$\pm$.01           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|}
                                                                      & GRintGRout  & .47$\pm$.05        & .43$\pm$.03             & .\textbf{82$\pm$.05} & .86$\pm$.04                & \textbf{.72$\pm$.03} & .73$\pm$.02             & {\cellcolor[rgb]{0.847,0.847,0.847}}.\textbf{76$\pm$.02} & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.79$\pm$.01} &  & .46$\pm$.03        & .41$\pm$.02             & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.82$\pm$.01} & {\cellcolor[rgb]{0.847,0.847,0.847}}.84$\pm$.01           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|}
                                                                      & LFintLFout  & .53$\pm$.03        & .46$\pm$.03             & .65$\pm$.10          & .83$\pm$.03                & .60$\pm$.09          & .68$\pm$.05             & {\cellcolor[rgb]{0.847,0.847,0.847}}.62$\pm$.10          & {\cellcolor[rgb]{0.847,0.847,0.847}}.74$\pm$.03          &  & .51$\pm$.01        & .45$\pm$.03             & {\cellcolor[rgb]{0.847,0.847,0.847}}.65$\pm$.12          & {\cellcolor[rgb]{0.847,0.847,0.847}}.81$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|}
                                                                      & GRintGRout+ & .46$\pm$.02        & .42$\pm$.01             & .76$\pm$.07          & \textbf{.88$\pm$.03}       & .71$\pm$.05          & .71$\pm$.06             & {\cellcolor[rgb]{0.847,0.847,0.847}}.73$\pm$.02          & {\cellcolor[rgb]{0.847,0.847,0.847}}.78$\pm$.02          &  & .45$\pm$.02        & .39$\pm$.02             & {\cellcolor[rgb]{0.847,0.847,0.847}}.81$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.85$\pm$.03}  \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|}
                                                                      & LFintLFout+ & .50$\pm$.02        & .43$\pm$.01             & .72$\pm$.09          & .86$\pm$.05                & .65$\pm$.02          & \textbf{.74$\pm$.02}    & {\cellcolor[rgb]{0.847,0.847,0.847}}.68$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.79$\pm$.02} &  & .49$\pm$.02        & .41$\pm$.03             & {\cellcolor[rgb]{0.847,0.847,0.847}}.75$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}.84$\pm$.01           \\
\hhline{|-|-|-|-|-|-|-|-|-|-|~|-|-|-|-|}
\end{tabular}
\end{table*}




==> tables/results0___.tex <==
% \usepackage{colortbl}
% \usepackage{multirow}
% \usepackage{hhline}

\begin{table*}
\footnotesize\addtolength{\tabcolsep}{-6pt}
\begin{center}
\caption{Domain Adaptation Results.}
\label{tab:results0} %https://tex.stackexchange.com/a/59805
%%%%%%%%%%%%%%%%%%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|} 
\cline{3-10}\cline{12-19}
\multicolumn{2}{c|}{\textbf{}}                                                      & \multicolumn{8}{c|}{\textbf{TestRc (classical \& funk)}}                                                                                                                                                                                                    &  & \multicolumn{8}{c|}{\textbf{TestRj (jazz)}}                                                                                                                                                                                                                  \\ 
\hhline{|--|--|--|--|--|~|--|--|--|--|}
\multicolumn{2}{|c|}{\textbf{Method}}                                               & \multicolumn{2}{c|}{\textbf{RMSE $\downarrow$}} & \multicolumn{2}{c|}{\textbf{Precision $\uparrow$}} & \multicolumn{2}{c|}{\textbf{Recall $\uparrow$}} & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{F1-Score $\uparrow$}}                          &  & \multicolumn{2}{c|}{\textbf{RMSE $\downarrow$}} & \multicolumn{2}{c|}{\textbf{Precision $\uparrow$}} & \multicolumn{2}{c|}{\textbf{Recall $\uparrow$}} & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{F1-Score $\uparrow$}}                           \\ 
\hhline{|-|-|--|--|--|--|~|--|--|--|--|}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Lower\\Bound\end{tabular}} & S           & \multicolumn{2}{c|}{.51$\pm$.01}                 & \multicolumn{2}{c|}{.80$\pm$.03}                    & \multicolumn{2}{c|}{.48$\pm$.03}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.60$\pm$.02}                                            &  & \multicolumn{2}{c|}{.45$\pm$.01}                 & \multicolumn{2}{c|}{.83$\pm$.02}                    & \multicolumn{2}{c|}{.51$\pm$.02}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.63$\pm$.01}                                             \\ 
\hhline{|~|-|--|--|--|--|~|--|--|--|--|}
                                                                      & S+          & \multicolumn{2}{c|}{.44$\pm$.00}                 & \multicolumn{2}{c|}{.84$\pm$.01}                    & \multicolumn{2}{c|}{.57$\pm$.01}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.68$\pm$.01}                                            &  & \multicolumn{2}{c|}{.40$\pm$.01}                 & \multicolumn{2}{c|}{.89$\pm$.01}                    & \multicolumn{2}{c|}{.62$\pm$.02}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.73$\pm$.02}                                             \\ 
\hhline{|-|-|--|--|--|--|~|--|--|--|--|}
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Upper\\Bound\end{tabular}} & R           & \multicolumn{2}{c|}{.34$\pm$.01}                 & \multicolumn{2}{c|}{.95$\pm$.03}                    & \multicolumn{2}{c|}{.71$\pm$.03}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.81$\pm$.01}                                            &  & \multicolumn{2}{c|}{.36$\pm$.01}                 & \multicolumn{2}{c|}{.93$\pm$.01}                    & \multicolumn{2}{c|}{.66$\pm$.03}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.77$\pm$.02}                                             \\ 
\hhline{|~|-|--|--|--|--|~|--|--|--|--|}
                                                                      & R\&S        & \multicolumn{2}{c|}{.33$\pm$.02}                 & \multicolumn{2}{c|}{.96$\pm$.03}                    & \multicolumn{2}{c|}{.71$\pm$.04}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.82$\pm$.02}                                            &  & \multicolumn{2}{c|}{.30$\pm$.01}                 & \multicolumn{2}{c|}{.98$\pm$.01}                    & \multicolumn{2}{c|}{.70$\pm$.06}                 & \multicolumn{2}{c|}{{\cellcolor[rgb]{0.847,0.847,0.847}}.81$\pm$.04}                                             \\ 
\cline{1-10}\cline{12-19}
\multicolumn{2}{|c|}{\textit{\textbf{Stopping Epoc}}h}                              & \textit{200th} & \textit{Sel.}               & \textit{200th}   & \textit{Sel.}                & \textit{200th}   & \textit{Sel.}             & \textit{200th}                                       & \textit{Sel.}                                        &  & \textit{200th} & \textit{Sel.}               & \textit{200th}   & \textit{Sel.}                & \textit{200th}   & \textit{Sel.}             & \textit{200th}                                       & \textit{Sel.}                                         \\ 
\hhline{|-|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Adv.\\Adap.\end{tabular}}  & GRint       & .48$\pm$.03        & .42$\pm$.02                     & .81$\pm$.05          & .86$\pm$.02                      & .57$\pm$.04          & .60$\pm$.04                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.67$\pm$.02          & {\cellcolor[rgb]{0.847,0.847,0.847}}.71$\pm$.02          &  & .45$\pm$.03        & .40$\pm$.01                     & .86$\pm$.04          & .92$\pm$.01                      & .59$\pm$.06          & .67$\pm$.04                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.70$\pm$.04          & {\cellcolor[rgb]{0.847,0.847,0.847}}.77$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                                                      & LFint       & .50$\pm$.03        & .46$\pm$.03                     & .71$\pm$.06          & .81$\pm$.04                      & .44$\pm$.09          & .53$\pm$.03                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.53$\pm$.08          & {\cellcolor[rgb]{0.847,0.847,0.847}}.64$\pm$.03          &  & .47$\pm$.01        & .46$\pm$.03                     & .79$\pm$.04          & .86$\pm$.04                      & .44$\pm$.13          & .57$\pm$.04                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.56$\pm$.12          & {\cellcolor[rgb]{0.847,0.847,0.847}}.69$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                                                      & GRout       & .51$\pm$.02        & .48$\pm$.01                     & .68$\pm$.02          & .78$\pm$.04                      & .67$\pm$.02          & .67$\pm$.04                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.67$\pm$.02          & {\cellcolor[rgb]{0.847,0.847,0.847}}.72$\pm$.03          &  & .51$\pm$.03        & .47$\pm$.01                     & .77$\pm$.03          & .84$\pm$.06                      & .75$\pm$.03          & .75$\pm$.04                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.76$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}.79$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                                                      & LFout       & .51$\pm$.02        & .47$\pm$.02                     & .64$\pm$.04          & .79$\pm$.04                      & .67$\pm$.02          & .68$\pm$.02                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.65$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}.73$\pm$.02          &  & .51$\pm$.03        & .46$\pm$.01                     & .71$\pm$.05          & .87$\pm$.03                      & .75$\pm$.04          & .74$\pm$.03                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.73$\pm$.04          & {\cellcolor[rgb]{0.847,0.847,0.847}}.80$\pm$.01           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                                                      & GRintGRout  & .47$\pm$.05        & .43$\pm$.03                     & \textbf{.82$\pm$.05} & .86$\pm$.04                      & \textbf{.72$\pm$.03} & .73$\pm$.02                   & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.76$\pm$.02} & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.79$\pm$.01} &  & .46$\pm$.03        & .41$\pm$.02                     & \textbf{.88$\pm$.03} & .91$\pm$.02                      & .77$\pm$.03          & .\textbf{79$\pm$.03}          & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.82$\pm$.01} & {\cellcolor[rgb]{0.847,0.847,0.847}}.84$\pm$.01           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                                                      & LFintLFout  & .53$\pm$.03        & .46$\pm$.03                     & .65$\pm$.10          & .83$\pm$.03                      & .60$\pm$.09          & .68$\pm$.05                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.62$\pm$.10          & {\cellcolor[rgb]{0.847,0.847,0.847}}.74$\pm$.03          &  & .51$\pm$.01        & .45$\pm$.03                     & .69$\pm$.12          & .88$\pm$.02                      & .61$\pm$.13          & .75$\pm$.04                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.65$\pm$.12          & {\cellcolor[rgb]{0.847,0.847,0.847}}.81$\pm$.03           \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                                                      & GRintGRout+ & .46$\pm$.02        & .42$\pm$.01                     & .76$\pm$.07          & \textbf{.88$\pm$.03}             & .71$\pm$.05          & .71$\pm$.06                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.73$\pm$.02          & {\cellcolor[rgb]{0.847,0.847,0.847}}.78$\pm$.02          &  & .45$\pm$.02        & .39$\pm$.02                     & .85$\pm$.06          & \textbf{.95$\pm$.02}             & \textbf{.78$\pm$.05} & .77$\pm$.05                   & {\cellcolor[rgb]{0.847,0.847,0.847}}.81$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.85$\pm$.03}  \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
                                                                      & LFintLFout+ & .50$\pm$.02        & .43$\pm$.01                     & .72$\pm$.09          & .86$\pm$.05                      & .65$\pm$.02          & \textbf{.74$\pm$.02}          & {\cellcolor[rgb]{0.847,0.847,0.847}}.68$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}\textbf{.79$\pm$.02} &  & .49$\pm$.02        & .41$\pm$.03                     & .80$\pm$.08          & .89$\pm$.03                      & .71$\pm$.03          & \textbf{.79$\pm$.01}          & {\cellcolor[rgb]{0.847,0.847,0.847}}.75$\pm$.03          & {\cellcolor[rgb]{0.847,0.847,0.847}}.84$\pm$.01           \\
\hhline{|-|-|-|-|-|-|-|-|-|-|~|-|-|-|-|-|-|-|-|}
\end{tabular}
%%%%%%%%%%%%%%%%%%
\begin{scriptsize}
\newline
\begin{flushright}
\vspace{-1.4em}
\textit{Sel.} is shorten from model selection; $\uparrow$/$\downarrow$ represent the higher/lower is better respectively.
\end{flushright}
\end{scriptsize}
\end{center}
\normalsize
\end{table*}


==> tables/results0a.tex <==
\begin{table}
\footnotesize\addtolength{\tabcolsep}{-6pt}
\begin{center}
\caption{Domain Adaptation Results on Additional Metrics}
\label{tab:results0a} %https://tex.stackexchange.com/a/59805
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\cline{3-8}
\multicolumn{2}{l|}{}                                                                       & \multicolumn{6}{c|}{\textbf{TestRc (classical \& funk)}}                                                                                       \\ 
\hline
\multicolumn{2}{|c|}{\textbf{\textit{Method}}}                                                       & \multicolumn{2}{c|}{\textbf{RMSE $\downarrow$}} & \multicolumn{2}{c|}{\textbf{Precision $\uparrow$}} & \multicolumn{2}{c|}{\textbf{Recall $\uparrow$}}  \\ 
\hline
Low B.                                                               & S                    & \multicolumn{2}{c|}{.51$\pm$.01}                 & \multicolumn{2}{c|}{.80$\pm$.03}                    & \multicolumn{2}{c|}{.48$\pm$.03}                  \\ 
\hline
Up B.                                                                & R                    & \multicolumn{2}{c|}{.34$\pm$.01}                 & \multicolumn{2}{c|}{.95$\pm$.03}                    & \multicolumn{2}{c|}{.71$\pm$.03}                  \\ 
\hline
\multirow{2}{*}{Others}                                              & R\&S                   & \multicolumn{2}{c|}{.33$\pm$.02}                 & \multicolumn{2}{c|}{.96$\pm$.03}                    & \multicolumn{2}{c|}{.71$\pm$.04}                  \\ 
\cline{2-8}
                                                                     & S+                   & \multicolumn{2}{c|}{.44$\pm$.00}                 & \multicolumn{2}{c|}{.84$\pm$.01}                    & \multicolumn{2}{c|}{.57$\pm$.01}                  \\ 
\hline
\multicolumn{2}{|c|}{\textit{\textbf{Stopping Epoch}}}                                      & \textit{200th}       & \textit{Sel.}         & \textit{200th}       & \textit{Sel.}            & \textit{200th}   & \textit{Sel.}              \\ 
\hline
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Adv.\\Adap.\end{tabular}} & GRint                & .48$\pm$.03              & .42$\pm$.02               & .81$\pm$.05              & .86$\pm$.02                  & .57$\pm$.04          & .60$\pm$.04                    \\ 
\cline{2-8}
                                                                     & LFint                & .50$\pm$.03              & .46$\pm$.03               & .71$\pm$.06              & .81$\pm$.04                  & .44$\pm$.09          & .53$\pm$.03                    \\ 
\cline{2-8}
                                                                     & GRout                & .51$\pm$.02              & .48$\pm$.01               & .68$\pm$.02              & .78$\pm$.04                  & .67$\pm$.02          & .67$\pm$.04                    \\ 
\cline{2-8}
                                                                     & LFout                & .51$\pm$.02              & .47$\pm$.02               & .64$\pm$.04              & .79$\pm$.04                  & .67$\pm$.02          & .68$\pm$.02                    \\ 
\cline{2-8}
                                                                     & GRintGRout           & .47$\pm$.05              & .43$\pm$.03               & \textbf{.82$\pm$.05}     & .86$\pm$.04                  & \textbf{.72$\pm$.03} & .73$\pm$.02                    \\ 
\cline{2-8}
                                                                     & LFintLFout           & .53$\pm$.03              & .46$\pm$.03               & .65$\pm$.10              & .83$\pm$.03                  & .60$\pm$.09          & .68$\pm$.05                    \\ 
\cline{2-8}
                                                                     & GRintGRout+          & \textbf{.46$\pm$.02}              &\textbf{ .42$\pm$.01}               & .76$\pm$.07              & \textbf{.88$\pm$.03}         & .71$\pm$.05          & .71$\pm$.06                    \\ 
\cline{2-8}
                                                                     & LFintLFout+          & .50$\pm$.02              & .43$\pm$.01               & .72$\pm$.09              & .86$\pm$.05                  & .65$\pm$.02          & \textbf{.74$\pm$.02}           \\ 
\hline
\multicolumn{1}{l}{}                                                 & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}  & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}     & \multicolumn{2}{l}{}                         
\end{tabular}

%%%%%%%%%%%%%%%%%%
\begin{scriptsize}
\begin{center}
\vspace{-2.4em}
\textit{Low B.}, \textit{Up B.}, \textit{Adv. Adap.}, and \textit{Sel.} is short for lower, upper bound, \\adversarial adaptation, and model selection respectively; \\$\uparrow$/$\downarrow$ represent the higher/lower is better respectively.
\end{center}
\end{scriptsize}
%%%%%%%%%%%%%%%%%%

\end{center}
\normalsize
\end{table}


==> tables/results0b.tex <==
\begin{table}
\footnotesize\addtolength{\tabcolsep}{-2pt}
\begin{center}
\caption{Comparison of F1-Score with/without Model Selection.}
\label{tab:results0b} %https://tex.stackexchange.com/a/59805

\begin{tabular}{ccccccc}\toprule

\multicolumn{2}{l}{}                                                              & \multicolumn{5}{c}{ \textbf{F1-Score $\uparrow$}}                                                                                                                                                               \\ 
\cmidrule{3-7}
\multicolumn{2}{c}{\textbf{\textit{Test Data}}}                                  & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{TestRc}\\\textbf{(classical\&funk)} \end{tabular}} &  & \multicolumn{2}{c}{\begin{tabular}[c]{@{}c@{}}\textbf{TestRj}\\\textbf{(jazz)}\end{tabular}}  \\ 
\multicolumn{2}{c}{\textit{\textbf{Stopping Epoch}}}                             & \textit{200th}   & \textit{Sel.}                                                                          &  & \textit{200th}   & \textit{Sel.}                                                               \\ 
\cmidrule{1-7}
\multirow{8}{*}{\begin{tabular}[c]{@{}c@{}}Adv.\\Adap.\end{tabular}} & GRint       & .67$\pm$.02          & .71$\pm$.02                                                                                &  & .70$\pm$.04          & .77$\pm$.03                                                                     \\ 

                                                                     & LFint       & .53$\pm$.08          & .64$\pm$.03                                                                                &  & .56$\pm$.12          & .69$\pm$.03                                                                     \\ 

                                                                     & GRout       & .67$\pm$.02          & .72$\pm$.03                                                                                &  & .76$\pm$.03          & .79$\pm$.03                                                                     \\ 

                                                                     & LFout       & .65$\pm$.03          & .73$\pm$.02                                                                                &  & .73$\pm$.04          & .80$\pm$.01                                                                     \\ 

                                                                     & GRintGRout  & \textbf{.76$\pm$.02} & \textbf{.79$\pm$.01}                                                                       &  & \textbf{.82$\pm$.01} & .84$\pm$.01                                                                     \\ 

                                                                     & LFintLFout  & .62$\pm$.10          & .74$\pm$.03                                                                                &  & .65$\pm$.12          & .81$\pm$.03                                                                     \\ 

                                                                     & GRintGRout+ & .73$\pm$.02          & .78$\pm$.02                                                                                &  & .81$\pm$.03          & \textbf{.85$\pm$.03}                                                            \\ 

                                                                     & LFintLFout+ & .68$\pm$.03          & \textbf{.79$\pm$.02}                                                                       &  & .75$\pm$.03          & .84$\pm$.01                                                                     \\
\bottomrule
\end{tabular}

%%%%%%%%%%%%%%%%%%
\begin{scriptsize}
\begin{center}
\vspace{-1.4em}
\textit{Adv. Adap.}, and \textit{Sel.} is short for adversarial adaptation, and model selection; %\\$\uparrow$ represent the higher is better.
\end{center}
\end{scriptsize}
%%%%%%%%%%%%%%%%%%



\end{center}
\normalsize
\end{table}

